High-Order Finite Element Second Moment Methods for Linear Transport

We present high-order, finite element-based Second Moment Methods (SMMs) for solving radiation transport problems in two spatial dimensions. We leverage the close connection between the Variable Eddington Factor (VEF) method and SMM to convert existing discretizations of the VEF moment system to discretizations of the SMM moment system. The moment discretizations are coupled to a high-order Discontinuous Galerkin discretization of the Discrete Ordinates transport equations. We show that the resulting methods achieve high-order accuracy on high-order (curved) meshes, preserve the thick diffusion limit, and are effective on a challenging multi-material problem both in outer fixed-point iterations and in inner preconditioned iterative solver iterations for the discrete moment systems. We also present parallel scaling results and provide direct comparisons to the VEF algorithms the SMM algorithms were derived from.

==> figs/vmms_1.tex <==
\begin{tabular}{cccccccccccc}
\toprule
 &  &  & \multicolumn{2}{c}{$\| \varphi - \varphi_\text{ex}\|$}  &  & \multicolumn{2}{c}{$\| \varphi - \Pi \varphi_\text{ex}\|$}  &  & \multicolumn{2}{c}{$\| \vec{J} - \vec{J}_\text{ex}\|$} \\
\cmidrule{4-5}\cmidrule{7-8}\cmidrule{10-11}
$p$ & $h$ & & RT & HRT & & RT & HRT & & RT & HRT \\
\midrule
\multirow{4}{*}{1} & \num{3.998e-02} & & \num{9.661e-04} & \num{9.661e-04} & & \num{1.343e-04} & \num{1.343e-04} & & \num{1.794e-02} & \num{1.794e-02} \\
 & \num{1.999e-02} & & \num{2.411e-04} & \num{2.411e-04} & & \num{2.867e-05} & \num{2.867e-05} & & \num{9.040e-03} & \num{9.040e-03} \\
 & \num{1.333e-02} & & \num{1.071e-04} & \num{1.071e-04} & & \num{1.207e-05} & \num{1.207e-05} & & \num{6.036e-03} & \num{6.036e-03} \\
 & \num{9.995e-03} & & \num{6.022e-05} & \num{6.022e-05} & & \num{6.612e-06} & \num{6.612e-06} & & \num{4.530e-03} & \num{4.530e-03} \\
\addlinespace
\multirow{4}{*}{2} & \num{5.880e-02} & & \num{8.299e-05} & \num{8.299e-05} & & \num{2.655e-05} & \num{2.655e-05} & & \num{4.792e-04} & \num{4.792e-04} \\
 & \num{3.029e-02} & & \num{1.147e-05} & \num{1.147e-05} & & \num{3.746e-06} & \num{3.746e-06} & & \num{8.953e-05} & \num{8.953e-05} \\
 & \num{1.999e-02} & & \num{3.307e-06} & \num{3.307e-06} & & \num{1.089e-06} & \num{1.089e-06} & & \num{3.149e-05} & \num{3.149e-05} \\
 & \num{1.492e-02} & & \num{1.376e-06} & \num{1.376e-06} & & \num{4.552e-07} & \num{4.552e-07} & & \num{1.511e-05} & \num{1.511e-05} \\
\addlinespace
\multirow{4}{*}{3} & \num{7.689e-02} & & \num{1.062e-05} & \num{1.062e-05} & & \num{1.809e-06} & \num{1.809e-06} & & \num{1.397e-04} & \num{1.397e-04} \\
 & \num{3.998e-02} & & \num{7.722e-07} & \num{7.722e-07} & & \num{1.080e-07} & \num{1.080e-07} & & \num{2.021e-05} & \num{2.021e-05} \\
 & \num{2.630e-02} & & \num{1.444e-07} & \num{1.444e-07} & & \num{1.845e-08} & \num{1.845e-08} & & \num{5.797e-06} & \num{5.797e-06} \\
 & \num{1.999e-02} & & \num{4.814e-08} & \num{4.814e-08} & & \num{5.901e-09} & \num{5.901e-09} & & \num{2.551e-06} & \num{2.551e-06} \\
\bottomrule
\end{tabular}
